Multicast-partitioning in Time-triggered Stream Planning for Time-Sensitive Networks

Multicast allows sending a message to multiple recipients without having to create and send a separate message for each recipient. This preserves network bandwidth, which is particularly important in time-sensitive networks. These networks are commonly used to provide latency-bounded communication for real-time systems in domains like automotive, avionics, industrial internet of things, automated shop floors, and smart energy grids. The preserved bandwidth can be used to admit additional real-time messages with specific quality of service requirements or to reduce the end-to-end latencies for messages of any type. However, using multicast communication can complicate traffic planning, as it requires free queues or available downstream egress ports on all branches of the multicast tree. In this work, we present a novel multicast partitioning technique to split multicast trees into smaller multicast or unicast trees. This allows for a more fine-grained trade-off between bandwidth utilization and traffic scheduling difficulty. Thus, schedulability in dynamic systems can be improved, in terms the number of admitted streams and the accumulated network throughput. We evaluated the multicast partitioning on different network topologies and with three different scheduling algorithms. With the partitioning, 5-15\% fewer streams were rejected, while achieving 5-125\% more network throughput, depending on the scheduling algorithm.

==> chapters/preliminaries.tex <==
% !TeX spellcheck = en_US
% !TeX root = ../cg_multicast_main.tex

% TODO das Kapitel braucht es in der neuen Struktur so nicht mehr. -> Fundamentals of scheduling denkbar/sinnvoll (TSN scheduling Synthesis), aber sollte dann zur Problemstellung. 
\section{Fundamentals of Conflict Graph-based Scheduling Synthesis}

In this section, we will provide a formal description of the scheduling synthesis problem in TSN, followed by an introduction to conflict graphs with a transformation from the scheduling synthesis solution space to a conflict graph.
Finally, we present the independent colorful set problem, a graph problem that can be used to formalize the search for a valid schedule in a conflict graph created by the transformation.

\subsection{TSN Scheduling Synthesis}
\label{sec:preliminaries:scheduling-problem}

A TSN schedule describes a timetable for every frame from all time-triggered streams in $\mathcal{S}$ that ensures that no two frames can collide, i.e., try to pass the same egress port on a bridge at the same time.
Two frames colliding can be avoided by either separating them spatially -- taking routes that do not overlap -- or temporally -- sending them time-delayed.
A stream's configuration can be described by its phase $\phi$ and route $\pi$.
Those two features and the streams properties allow for a deterministic description of the time resources are required by a stream.
Assume that the route $\pi$ is a path in $\mathcal{N}$ and $tx_\pi(f, [u, v])$ denotes the transmission interval of frame $f$ requires on the egress port leading from network device $u$ to device $v$ if it is sent at time $\phi$ of its stream within the frames cycle.
In case of multicasts $\pi$ represents a tree in $\mathcal{N}$, while $tx_\pi(f, [u, v])$ remains unchanged.
Further, let $\mathcal{F}(s)$ be the set of frames belonging to stream $s$ within a hypercycle. 

A valid schedule assigns $\phi$ and $\pi$ so that

\begin{equation}
	\begin{split}
		& \forall s_1, s_2 \in \mathcal{S}, s_1 \neq s_2, f_1 \in \mathcal{F}(s_1), f_2 \in \mathcal{F}(s_2): \\
		& \forall [u, v] \in \pi_1 \cap \pi_2: \\
		& tx_{\pi_1}(f_1, [u, v])~\neg \text{ overlap } tx_{\pi_2}(f_2, [u, v])
	\end{split}
\end{equation}

Or in simple words: $\pi$ and $\phi$ have to be chosen for all streams so that no two frames collide, i.e., their transmission overlaps, at any egress port.
In case there is no valid schedule (or the heuristic does not find it) the goal is to admit as many streams as possible.


\subsection{Conflict Graph Modeling}

A conflict graph $\mathcal{G_C}$ is an undirected vertex colored graph $(\mathcal{V, E, C})$ with the vertex set $\mathcal{V}$, the set of undirected edges $\mathcal{E} \subseteq \mathcal{V}^2$, and the set of colors $\mathcal{C}$ \cite{Geppert2024}.
Each vertex $v \in \mathcal{V}$ can be mapped to a single color $c \in \mathcal{C}$ with the surjective function $col(v): \mathcal{V} \mapsto \mathcal{C}$.

We can model the solution space to the scheduling synthesis problem as a conflict graph.
Therefore, we $\mathcal{V}$ is the set of possible stream configurations, $\mathcal{E}$ connects mutual exclusive configurations, and $\mathcal{C}$ denotes the set of streams.
Hence, every stream is represented by a color.
A configuration (or vertex) $v$ represents a specific combination of $\pi$ and $\phi$ for its stream $S = col(v)$.
If the configurations two streams are not compatible, meaning their frames would collide eventually, the configurations are connected with an edge.
This way, we can model the whole solution space, i.e., all possible $\pi-\phi$--combinations for every stream.
This would result in a huge conflict graph even for medium-sized scheduling problems.
However, the conflict graph model can also be used to model a partial solution space, e.g., only a fraction of the possible $\pi-\phi$--combinations for every stream.
This allows for faster heuristic solutions or additional constraints such as QoS guarantees when updating schedules \cite{Falk2022}.



\subsection{Scheduling Synthesis via Conflict Graphs}

We can use the notion of an \emph{independent colorful set} (ICS) to create a TSN schedule from a conflict graph $\mathcal{G_C}$.
An independent colorful set describes an extension to the independent set (IS) that describes a subset of vertices in a graph $\mathcal{G}$ that are not directly connected:

\begin{equation}
	\label{eq:prelim:is}
	IS(\mathcal{G}) \subseteq \mathcal{V} \mid \forall v_i, v_j \in IS, i \neq j: (v_i, v_j) \notin \mathcal{E}
\end{equation}

The maximum independent subset problem denotes the challenge of finding an IS of maximum size.
Now, an independent colorful set denotes an independent set where each member has a distinct color:

\begin{equation}
	\label{eq:prelim:ics}
	\begin{split}
		ICS(\mathcal{G_C}) = & \max IS(\mathcal{G}_\mathcal{C}) \mid \\
		& \forall v_i, v_j \in IS, i~\neq~j:  col(v_i) \neq col(v_j)	
	\end{split}
\end{equation}

An ICS from a conflict graph $\mathcal{G_C}$ as described in the previous subsection is a set of stream configurations where no two streams will have colliding frames.
Hence, it describes a valid schedule for the TSN scheduling problem.
If the ICS is tropical, i.e., it  contains a vertex of every color in $\mathcal{C}$ \cite{d2018tropical}, it represents a schedule where each stream has a valid assignment.
A tropical ICS can be found in a subset of the whole solution space. 
Thus, a smaller $\mathcal{G_C}$ can still hold an optimal solution, which is beneficial since smaller conflict graphs need less memory and can be created much faster \cite{Geppert2024}.

